Static Race Detection for RTOS Applications

We present a static analysis technique for detecting data races in Real-Time Operating System (RTOS) applications. These applications are often employed in safety-critical tasks and the presence of races may lead to erroneous behaviour with serious consequences. Analyzing these applications is challenging due to the variety of non-standard synchronization mechanisms they use. We propose a technique based on the notion of an "occurs-in-between" relation between statements. This notion enables us to capture the interplay of various synchronization mechanisms. We use a pre-analysis and a small set of not-occurs-in-between patterns to detect whether two statements may race with each other. Our experimental evaluation shows that the technique is efficient and effective in identifying races with high precision.

==> app-soundness.tex <==
\section{Soundness of the conditions}
\label{sec:app-soundness}

We sketch here a proof of Thm.~\ref{thm:noib-soundness} on the
soundness of the conditions C1--C6.
Let $P$ be an IDA program with statements $s_1$ and $s_2$ satisfying
one of the conditions C1--C6. We need to argue that in each case $s_1
\noibsymb s_2$.
We focus on the first three rules C1--C3 since the remaining are more
standard and their soundness is easy to see.

\textbf{C1:}
Suppose $s_1$ and $s_2$ satisfy the condition C1, and suppose there is
an execution $\rho$ of $P$ in which $s_2$ occurs in between $s_1$.
Let us say $s_1$ is executed by thread $t_1$ and $s_2$ by thread $t_2$.
Then $s_2$ must happen some time after $t_2$ was suspended by
$t_1$, and before $s_1$ takes place.
The only way this can happen is if:
\begin{itemize}
\item Some thread $t_3$ with priority
\emph{greater than or equal to} $p_1$ resumes $t_2$.
But this is not possible since the condition says that there is \emph{no} other
task with dynamic priority greater than or equal to $p_1$ which can
resume $B$.
    \item $t_1$ makes a blocking call and another task runs and
      resumes $t_2$. However this is ruled out by the requirement that
      [there is no \block\ command before $s_{1}$] OR [there is no
        task other than $A$ which can resume $B$].
\end{itemize}

\smallskip
\textbf{C2:}
Suppose $s_1$ and $s_2$ satisfy the condition C2, and suppose there is
an execution $\rho$ of $P$ in which $s_2$ occurs in between $s_1$.
Let us say $s_1$ is executed by thread $t_1$ and $s_2$ by thread $t_2$.
Then thread $t_2$ must preempt thread $t_1$ during the execution of $s_1$.
The only way this can happen is if:
\begin{itemize}
\item $t_2$ with priority
\emph{greater than} $p_1$ was blocked. It runs and preempts $t_1$.
But this is not possible since the condition says that $p_{1}$ $>$ maximum dynamic priority of $t_2$.
\item $t_2$ has a priority
\emph{equal to} $p_1$ and $t_1$'s time slice expires and it gets
preempted by $t_2$.
Again, this is not possible since the condition says that $p_{1}$ $>$ maximum dynamic priority of $t_2$.
\item Some thread $t_3$ with priority
\emph{greater than or equal to} $p_1$ was blocked. It runs and suspends $t_1$. However this is ruled out by the requirement that
there is no task other than $t_1$ with maximum dynamic priority $\geq$ $p_1$, which can suspend $t_1$.
\end{itemize}

\smallskip
\textbf{C3:}
Suppose $s_1$ and $s_2$ satisfy the condition C3, and suppose there is
an execution $\rho$ of $P$ in which $s_2$ occurs in between $s_1$.
Let us say $s_1$ is executed by thread $t_1$ and $s_2$ by thread $t_2$.
Then $s_2$ must happen some time after $flag_1$ is set to 1 by $t_1$, and before $s_1$ takes place.
The only way this can happen is if:
\begin{itemize}
\item Some thread $t_3$ with priority
\emph{greater than or equal to} $p_1$ was blocked. It runs and resets $flag_1$ to 0. But this is not possible since the condition says that 
$s_1$ is either in the scope of a \suspendsched\ command or there is no thread of priority $\geq$ $p_1$ that resets $flag_1$.
\item $t_1$ makes a blocking call and another task runs and resets $flag_1$ to 0.
Again, this is not possible because of the requirement that [there is no \block\ command before $s_1$] OR [there is no task other than $t_1$ which can reset $flag_1$ to 0].
\item Both $t_1$ and $t_2$ run at the same priority. Before $t_1$ sets $flag_1$ to 1, $t_2$ checks $flag_1$ and finds that it is 0, and enters the block containing $s_2$. Before $t_2$ executes $s_2$, it's time slice expires. It gets preempted by $t_1$ which sets $flag_1$ to 1 and starts $s_1$. However this is ruled out by the requirement that $p_2$ $>$  $p_1$.
\end{itemize}

This completes the argument.
\qed


==> prod-cons-freertos.tex <==
void main(...) {                  Prio  Susp 
1. item = count = 0;              
2. xTaskCreate(prod,...,1, t1); 
3. xTaskCreate(cons,...,1, t2); 
4. vTaskStartScheduler(); 
}

void prod(...) {
10. for( ; ; ) {                   1,1  -
11.   vTaskSuspend(t2);            1,1  -
12.   item = 5;                    1,1  cons
13.   count = count+1;             1,1  cons
14.   vTaskResume(t2);             1,1  cons
15. }                              1,1  -
}

void cons(...) {
20. for( ; ; ) {                   1,1  -
21.   temp = item;                 1,1  -   
22.   vTaskPrioritySet(NULL, 2);   1,1  -   
23.   count = count-1;             2,2  -  
24.   vTaskPrioritySet(NULL, 1);   2,2  -
25. }                              1,1  -
}

